Embedded minimal disks

This is a survey of our work on embedded minimal disks.

==> blow7 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1500 900 309 309 1500 900 1425 600
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1500 900
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 937 1447 870 1237
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 742 645 795 862
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 7
	 750 900 1125 975 1500 900 1650 825 1725 750 1950 525
	 2100 450
	 0.000 1.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 9
	 750 1275 750 1200 975 1125 1200 1050 1575 900 1725 825
	 1875 825 2025 750 2100 900
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
4 0 0 100 0 0 12 0.0000 2 195 870 931 1620 $\\Sigma_1$\001
4 0 0 100 0 0 12 0.0000 2 195 870 676 593 $\\Sigma_2$\001


==> blow8 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 2243 982 375 375 2243 982 2543 757
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 757 1215 375 375 757 1215 1057 990
1 2 0 1 7 0 100 0 4 0.000 1 0.3491 920 1150 150 290 770 1150 1070 1150
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 757 1222
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2243 982
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1545 1192 1387 1043
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 11
	 3075 300 2625 825 1950 900 1275 900 825 225 600 1125
	 1125 1875 1500 1050 2250 975 2700 975 3150 1350
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 1 0 3
	0 0 1.00 60.00 120.00
	 915 1762 1043 1522 1005 1252
	 0.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 675 848 1965 $B_x^+$\001
4 0 0 100 0 0 12 0.0000 2 165 405 1477 1088 $\\nn$\001
4 0 0 100 0 0 12 0.0000 2 165 270 608 1364 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 270 2213 1170 $y$\001
4 0 0 100 0 0 12 0.0000 2 195 690 1342 720 $\\Sigma$\001


==> blow9 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
5 1 0 1 0 7 100 0 -1 0.000 0 0 0 0 862.500 937.500 1050 750 1125 975 1050 1125
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2400 360 2070 442
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 735 1417 802 1163
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 900 892
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 900 892 1050 757
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 892 892 1050 1125
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 6
	 1060 750 1110 705 1160 670 1305 570 1490 550 1950 365
	 0.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1060 1135 1145 1215 1355 1335 1595 1405 2000 1480
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 7
	 1955 360 2055 515 2140 740 2175 1035 2155 1265 2110 1430
	 1995 1485
	 0.000 1.000 1.000 1.000 1.000 1.000 0.000
3 0 1 1 0 7 100 0 -1 4.000 0 0 0 7
	 1058 757 975 615 802 667 607 727 622 937 825 1148
	 1058 1125
	 0.000 1.000 1.000 1.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 1560 2430 396 $\\partial \\cB_{r+R}$\001
4 0 0 100 0 0 12 0.0000 2 195 1155 616 1596 $\\partial \\cB_r$\001
4 0 0 100 0 0 12 0.0000 2 195 1410 1426 929 $S_{R}(\\gamma)$\001
4 0 0 100 0 0 12 0.0000 2 195 765 998 950 $\\gamma$\001


==> dis10 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
5 1 0 3 0 7 100 0 -1 0.000 0 0 0 0 866.071 1301.786 750 525 1425 750 1650 1350
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 750 1500 750 300
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 600 1350 2700 1350
4 0 0 100 0 0 12 0.0000 2 195 270 900 375 $y$\001
4 0 0 100 0 0 12 0.0000 2 165 270 2400 1575 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 2130 1575 600 $\\partial \\tilde{D}_r \\cap Q$\001


==> dis12 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1050 1275 1275 1500
2 2 0 1 0 0 100 0 4 0.000 0 0 -1 0 0 5
	 1350 600 2250 600 2250 1800 1350 1800 1350 600
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1050 1200 2175 1200
3 0 0 1 0 7 100 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 2700 825 2475 375 2025 375 1950 525
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 2700 1575 2400 2100 2100 2100 1950 1875
	 0.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 135 405 2400 1050 Short\001
4 0 0 100 0 0 12 0.0000 2 180 825 2400 1275 connecting\001
4 0 0 100 0 0 12 0.0000 2 90 555 2400 1500 curves.\001
4 0 0 100 0 0 12 0.0000 2 180 660 450 1050 Spiraling\001
4 0 0 100 0 0 12 0.0000 2 90 555 450 1275 curves.\001


==> dis19 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 675 675 225 1800 675 1125 450
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1725 675 225 1800 1725 1125 1500
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 675 2475 1725
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 1725 2475 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2400 375 2175 600
4 1 0 100 0 0 12 0.0000 2 165 270 1950 1275 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 1515 2272 323 $\\cone_{\\delta}(x)$\001


==> dis20 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1888 1465 169 169 1888 1465 2058 1465
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1076 1495 365 365 1076 1495 1441 1495
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 975 2175 2801 755
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1888 1465
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 975 755 2801 2175
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1888 1465
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 1970 1465 2294 1465 2598 1363 3106 1465
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 536 1573 873 1566 1178 1465 1483 1566 1800 1465
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 709 1466 975 1458 1178 1390 1440 1450
	 0.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 900 614 2003 $B_{s}(y)$\001
4 0 0 100 0 0 12 0.0000 2 195 900 1664 1822 $B_{2r_0}$\001
4 0 0 100 0 0 12 0.0000 2 195 750 893 1388 $\\Sigma'$\001
4 0 0 100 0 0 12 0.0000 2 195 870 2872 1642 $\\Sigma_d$\001
4 0 0 100 0 0 12 0.0000 2 195 1695 2453 637 $\\cone_{\\delta_0}(0)$\001


==> dis22 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1200 900 900 1800 1200 2700 1200
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1500 900 225 225 1500 900 1725 900
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1800 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 3
	 1492 900 1163 563 1170 570
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 502 990 1230 697
4 0 0 100 0 0 12 0.0000 2 195 1050 2407 2078 $B_{r_0}(x)$\001
4 0 0 100 0 0 12 0.0000 2 195 720 1725 750 $B_s(y)$\001
4 0 0 100 0 0 12 0.0000 2 165 270 1814 1402 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 270 1386 1035 $y$\001
4 0 0 100 0 0 12 0.0000 2 195 915 75 1200 $r_0 - r(y)$\001


==> dis27 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 3 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 6
	 1205 1707 1868 1035 3221 1040 2539 1714 1201 1710 1205 1707
2 3 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 6
	 1209 1260 1872 590 3225 594 2542 1269 1205 1264 1209 1260
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 44.97 89.93
	 3165 870 2228 997
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 791 486 982 780
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 15
	 2280 870 1120 842 614 884 469 935 415 1007 424 1058
	 460 1097 598 1136 686 1152 850 1152 949 1152 1030 1156
	 1093 1156 1256 1156 1311 1156
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 0.000
3 0 1 1 0 7 100 0 -1 4.000 0 0 0 3
	 1320 1148 1717 1177 2265 1207
	 0.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 135 795 3163 848 ``Between\001
4 0 0 100 0 0 12 0.0000 2 135 915 3262 1012 the sheets''\001
4 0 0 100 0 0 12 0.0000 2 135 360 600 458 Axis\001


==> dis4 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2258 1237 3112 1245
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2265 1155 3097 1155
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 2310 1170 2318 1260
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2812 360 3075 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2025 1725 2272 1290
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 9
	 3127 1245 2577 1640 1830 1725 861 1535 531 1136 982 722
	 1848 618 2733 755 3097 1148
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 9
	 2250 1234 2078 1337 1831 1365 1511 1302 1402 1170 1551 1033
	 1837 999 2130 1044 2273 1159
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
4 0 0 100 0 0 12 0.0000 2 195 3075 750 1950 Separation $w(1,0)$ over $\\partial D_1$.\001
4 0 0 100 0 0 12 0.0000 2 195 5310 825 225 $\\frac{c_1}{\\log \\rho} \\leq \\frac{w(\\rho,0)}{w(1,0)} \\leq c_2 \\log \\rho$\001


==> dis5 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 900 1950 900 300
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 450 1200 2700 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 817 1260 2145 690
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 810 1410 2145 855
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1267 1732 2115 1335
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1578 1805 2123 1567
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1815 1912 2108 1770
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 810 1095 2138 502
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 810 945 2160 345
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2160 90 2160 2198
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1043 2198 1275 1897
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2475 817 2198 1133
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 277 1801 652 1636
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 750 450 750 1800
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 844 1563 2097 1024
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1058 1665 2065 1182
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 2160 172 885 583 450 1200 885 1783 2160 2070
	 0.000 1.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 780 2400 1425 $\\log \\rho$\001
4 0 0 100 0 0 12 0.0000 2 195 2520 555 2392 $c |\\theta| = (1+ \\log \\rho)^{3/2}$\001
4 0 0 100 0 0 12 0.0000 2 195 615 2370 758 $\\log R$\001
4 0 0 100 0 0 12 0.0000 2 195 690 75 2025 $-\\log 2$\001
4 0 0 100 0 0 12 0.0000 2 165 615 945 300 $\\theta$\001


==> dis6 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 1320 225 3825 1950
1 4 0 1 0 7 100 0 -1 0.000 1 0.0000 2370 1200 750 750 1620 1200 3120 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1620 1950 1620 300
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1320 1200 3420 1200
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 1320 1800 1320 525
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2370 1200
4 0 0 100 0 0 12 0.0000 2 195 270 1695 375 $y$\001
4 0 0 100 0 0 12 0.0000 2 165 270 3270 1425 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 1005 2820 525 $D_{|x|}(x)$\001
-6
4 0 0 100 0 0 12 0.0000 2 195 1050 150 1253 $x\\leq-\\log 2$\001


==> dis8 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1799 1117 653 654 1799 1117 2452 1109
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1146 1092 1692 1090
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1155 1036 1690 1036
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1921 1092 2456 1092
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1913 1092 2449 1092
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1159 983 1692 983
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1905 1037 2449 1036
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1159 1222 1692 1222
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1151 1163 1687 1163
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1898 1282 2429 1282
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1898 1215 2433 1215
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1905 1149 2449 1146
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 592 1702 1125 1170
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 42.01 84.02
	 2605 1479 2334 1342
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1035 375 1792 945
3 2 1 1 0 7 100 0 -1 2.000 0 0 0 3
	 1690 1036 1812 1008 1913 1036
	 0.000 -1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 870 442 1919 $\\Sigma_2$\001
4 0 0 100 0 0 12 0.0000 2 195 870 2677 1582 $\\Sigma_1$\001
4 0 0 100 0 0 12 0.0000 2 195 4185 600 300 $\\sigma_{\\theta} \\subset \\Sigma$ is a curve connecting\001
4 0 0 100 0 0 12 0.0000 2 135 1155 1965 472 the two halves.\001


==> dis9 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 1200 3000 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 1050 3000 1050
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 900 3000 900
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 750 3000 750
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 525 3000 525
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 1125 3000 1125
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 1275 3000 1275
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1200 1320 3000 1320
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1342 3517 1350
3 0 0 1 0 7 100 0 -1 0.000 0 1 1 4
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 1125 548 967 697 967 1140 1133 1297
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 3
	 3052 533 3172 637 3060 727
	 0.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 180 465 420 1020 height\001
4 0 0 100 0 0 12 0.0000 2 135 435 3202 697 Initial\001
4 0 0 100 0 0 12 0.0000 2 180 795 3105 892 separation\001
4 0 0 100 0 0 12 0.0000 2 135 435 419 825 Initial\001


==> loc1 <==
#FIG 3.2
Portrait
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1425 2850 1425
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1415 2850 1415
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1425 2850 1425
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3150 1200 2925 1425
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2175 2175 2100 1950
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 1650 1425 1650 2100
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1650 1425 1650 300
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 450 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 450 1275
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1125 1650 1125
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1275 1650 1275
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1915 1650 1915
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1655 1650 1655
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1500 1650 1500
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1435 1650 1435
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1385 1650 1385
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1650 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1650 1275
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 935 2850 935
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1195 2850 1195
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1350 2850 1350
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1725 2850 1725
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1575 2850 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1435 2850 1435
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1465 2850 1465
2 1 0 2 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1385 2850 1385
2 1 0 2 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1465 1650 1465
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 935 1650 935
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1125 2850 1125
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1195 1650 1195
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1275 2850 1275
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1350 1650 1350
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1915 2850 1915
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1725 1650 1725
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1655 2850 1655
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 450 1575 1650 1575
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1650 1500 2850 1500
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 750 675 600 900
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 750 2175 600 1950
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2252 646 2102 871
4 0 0 100 0 0 12 0.0000 2 195 1065 750 600 $\\Sigma_1^+$\001
4 0 0 100 0 0 12 0.0000 2 195 1065 810 2355 $\\Sigma_2^-$\001
4 0 0 100 0 0 12 0.0000 2 195 1065 2197 2363 $\\Sigma_1^-$\001
4 0 0 100 0 0 12 0.0000 2 195 735 3179 1163 $x_3 = 0$\001
4 0 0 100 0 0 12 0.0000 2 195 870 1710 382 $x_3$-axis\001
4 0 0 100 0 0 12 0.0000 2 195 1065 2317 683 $\\Sigma_2^+$\001


==> pl2a <==
#FIG 3.2
Portrait
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1500 300 75 1800 1500 1500 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1800 2100 1800 750
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2100 1125 1275 2175
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 600 1500 3000 1500
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 600 1500 3000 1500
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 2850 975 2475 1125 2175 1350 2100 1500
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 750 975 1125 1125 1425 1350 1500 1500
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 750 2025 1125 1875 1425 1650 1500 1500
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 2850 2025 2475 1875 2175 1650 2100 1500
	 0.000 -1.000 -1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 450 1875 750 $x_3$\001
4 0 0 100 0 0 12 0.0000 2 195 450 1425 2250 $x_1$\001
4 0 0 100 0 0 12 0.0000 2 195 450 2925 1725 $x_2$\001


==> shn3 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 1350 525 2351 1350
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2085 1262
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1762 1144 1674 1320
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1939 1144 2027 1291
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 879 1703 1144
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 850 2027 1115
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1821 908 1467 1057
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 800 2027 554
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 1 2
	0 0 1.00 28.86 57.71
	 1467 879 1851 730
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 760 1585 642
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1615 1133 1454 1213
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 2106 1075 2233 1144
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 818 2321 818
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 818 2262 683
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1851 840 2214 996
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1851 879 1851 730
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 2203 1005 2310 1027
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 28.86 57.71
	 1791 908 1380 908
3 2 1 1 0 7 100 0 -1 4.000 0 0 0 8
	 2321 818 2262 672 2145 584 2027 554 1821 554 1615 613
	 1467 760 1467 879
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 0.000
3 2 1 1 0 7 100 0 -1 4.000 0 0 0 11
	 1467 760 1418 798 1390 870 1399 967 1517 1084 1703 1144
	 1909 1144 2096 1084 2243 967 2311 879 2321 818
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 0.000
3 2 1 1 0 7 100 0 -1 4.000 0 0 0 13
	 1415 1005 1384 1046 1380 1093 1399 1163 1527 1268 1703 1320
	 1909 1320 2085 1262 2233 1144 2310 1026 2327 967 2332 879
	 2313 859
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 -1.000 0.000
-6
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1140 1920 1552 1350
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 6
	 1372 1095 1170 1163 930 1185 667 1432 405 1417 435 1425
	 0.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 12
	 412 1425 382 1627 1080 1755 1695 1755 2407 1530 2865 1305
	 2985 1050 2917 570 2213 195 1410 210 533 697 480 1148
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 1365 907 1005 945 652 1065 487 1133
	 0.000 1.000 1.000 0.000
4 0 0 100 0 32 12 0.0000 4 135 105 2482 1792 S\001
4 0 0 100 0 0 12 0.0000 2 180 2460 412 2108 Small multi-valued graph near 0.\001


==> shn5 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 2377 1023 2977 1335
1 2 0 1 0 7 100 0 -1 0.000 1 0.0000 2677 1075 300 52 2977 1127 2377 1023
1 2 0 1 0 7 100 0 -1 0.000 1 0.0000 2677 1283 300 52 2977 1335 2377 1231
1 2 0 1 0 7 100 0 -1 0.000 1 0.0000 2677 1178 225 27 2902 1205 2452 1152
-6
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1927 1170 1095 1095 1927 1170 3022 1170
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3217 675 2715 1050
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3210 1702 2715 1297
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3217 1170 2940 1170
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2670 1275
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2685 1080
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 9
	 2685 1073 2385 1073 2138 1065 1837 975 1612 1148 1845 1342
	 2153 1267 2392 1282 2670 1275
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 0.000
4 0 0 100 0 0 12 0.0000 2 195 930 3241 1230 $\\Sigma_3'$\001
4 0 0 100 0 0 12 0.0000 2 195 870 2429 884 $\\Sigma_1$\001
4 0 0 100 0 0 12 0.0000 2 195 870 2430 1589 $\\Sigma_2$\001
4 0 0 100 0 0 12 0.0000 2 195 450 3240 1808 $y_2$\001
4 0 0 100 0 0 12 0.0000 2 195 450 3248 660 $y_1$\001
4 0 0 100 0 0 12 0.0000 2 195 1125 2670 2213 $B_{c_1 r_0}$\001
4 0 0 100 0 0 12 0.0000 2 195 765 1672 1523 $\\gamma$\001


==> uls17 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1575 1125 503 503 1575 1125 1800 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1702 367 1590 825
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 630 1028 2670 1028
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1582 900
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 607 1155 847 1185 1163 1177 1492 1163
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 1680 1155 1905 1185 2273 1163 2677 1163
	 0.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 480 1455 1807 $B_1$\001
4 0 0 100 0 0 12 0.0000 2 195 915 435 960 $x_3 = c_0$\001
4 0 0 100 0 0 12 0.0000 2 195 1140 2482 1358 $\\Sigma_{d,i}$\001
4 0 0 100 0 0 12 0.0000 2 180 1185 1777 405 Point with large\001
4 0 0 100 0 0 12 0.0000 2 195 1815 1777 592 curvature in $\\Sigma_i$.\001


==> uls5 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1575 1200 839 839 1575 1200 2414 1200
1 3 0 1 0 7 100 0 -1 0.000 1 6.0039 1575 1200 309 309 1575 1200 1884 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2422 675 1672 1110
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2422 1942 1605 1252
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 7
	 750 975 1226 1145 1607 1177 1772 1146 1865 1095 2143 940
	 2385 952
	 0.000 1.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 9
	 742 1350 804 1259 1041 1249 1277 1238 1679 1198 1844 1167
	 1989 1208 2153 1282 2400 1425
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
4 0 0 100 0 0 12 0.0000 2 180 420 2475 675 graph\001
4 0 0 100 0 0 12 0.0000 2 180 420 2452 1972 graph\001


==> unot1 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2655 1297 1965 1552
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1665 2018 1665 68
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1468 3090 2393
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1443 2490 2468
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1418 1965 2468
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1393 1215 2318
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1368 840 2168
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1343 540 1943
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1318 240 1643
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1665 1493 3390 2318
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1293 165 1118
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1268 315 818
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1665 1243 540 668
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2212 1738 2437 1663
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2917 2077 3142 2002
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 11
	 2565 1943 2415 1943 2040 1868 1740 1793 1515 1643 1440 1568
	 1365 1493 1365 1343 1440 1268 1515 1193 1590 1193
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 135 1320 2166 1237 One half rotation.\001
4 0 0 100 0 0 12 0.0000 2 195 870 1792 300 $x_3$-axis\001


==> unot10 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 675 675 225 1800 675 1125 450
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1725 675 225 1800 1725 1125 1500
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1200 175 175 1800 1200 1975 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 1725 2475 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2362 1245 1875 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2362 1320 1505 1760
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1425 1800
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1800 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 675 2475 1725
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1800 1200
4 0 0 100 0 0 12 0.0000 2 195 270 1530 1890 $y$\001
4 0 0 100 0 0 12 0.0000 2 165 270 1643 1267 $0$\001
4 0 0 100 0 0 12 0.0000 2 195 1515 1545 706 $\\cone_{\\delta}(0)$\001
4 0 0 100 0 0 12 0.0000 2 195 1665 1253 1238 $B_{ \\frac{Cs}{2} }$\001
4 0 0 100 0 0 12 0.0000 2 135 945 2422 1260 Consecutive\001
4 0 0 100 0 0 12 0.0000 2 180 1140 2423 1417 blow up points.\001


==> unot11 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1882 1148 2460 1357
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1350 2400 1125 2175
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2550 1425
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1050 2100
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1567 1830
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1815 1747
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2025 1680
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2017 1900 1858 1794
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1965 1925 1626 1847
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2085 1900 2035 1700
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 975 2100 900 2175 750 2250 600 2250
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1125 2100 1425 2175 1800 2250 2475 2325 3000 2325
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 2475 1425 2325 1500 2250 1500 2100 1575 675 1425
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 3
	 2625 1425 2850 1500 3000 1500
	 0.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 180 2895 750 2550 Blow up point satisfying \\eqr{e:pairs}.\001
4 0 0 100 0 0 12 0.0000 2 180 2895 750 1050 Blow up point satisfying \\eqr{e:pairs}.\001
4 0 0 100 0 0 12 0.0000 2 180 3120 833 2035 Blow up points satisfying \\eqr{e:defc1ii}.\001


==> unot12 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2400 1425
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1575 2475 1275 2325
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1796 1653 1609 1448
2 1 1 1 0 7 100 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3675 2025 3675 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2100 1100 2375 1300
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 2400 1350
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1575 1425
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1200 2250
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 4
	 1125 2250 900 2250 750 2250 600 2325
	 0.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1275 2250 1500 2325 1800 2250 2475 2325 3000 2400
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 2325 1350 2250 1350 2175 1350 1875 1350 600 975
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 3
	 2475 1350 2850 1275 3000 1200
	 0.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1499 1360 1199 1320 1049 1360 824 1365 599 1360
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1649 1358 1950 1425 2250 1425 2924 1433 2999 1433
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 1500 1550 1200 1573 1050 1573 825 1498 600 1448
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 6
	 1650 1520 1876 1500 2176 1500 2550 1500 2851 1485 3000 1475
	 0.000 1.000 1.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 180 3030 675 1800 Blow up point satisfying \\eqr{e:defc1ii}.\001
4 0 0 100 0 0 12 0.0000 2 180 2895 750 2625 Blow up point satisfying \\eqr{e:pairs}.\001
4 0 0 100 0 0 12 0.0000 2 180 465 3450 1575 height\001
4 0 0 100 0 0 12 0.0000 2 180 2250 1125 900 The height of its multi-valued\001
4 0 0 100 0 0 12 0.0000 2 180 1335 1125 1050 graph could grow.\001
4 0 0 100 0 0 12 0.0000 2 180 2580 675 1950 The separation of its multi-valued\001
4 0 0 100 0 0 12 0.0000 2 180 2280 675 2100 graph could decay sublinearly.\001
4 0 0 100 0 0 12 0.0000 2 180 2895 1125 750 Blow up point satisfying \\eqr{e:pairs}.\001


==> unot2a <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 1091 2300
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1878 2014 2093 2443
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1449 2014 1234 2372
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1370 2022 2014
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1298 1234 1942
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1735 1442 2594 1799
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1179 1234 583
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 1 2
	0 0 1.00 57.25 114.51
	 2594 1370 1664 1012
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1084 2308 797
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 2236 1990 2609 2208
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1043 1847 733 2014
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 57.25 114.51
	0 0 1.00 57.25 114.51
	 2601 2229 2594 1799
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1227 518 1227
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1227 662 893
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1275 781 1656
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1664 1370 1664 225
2 1 1 1 0 7 100 0 -1 4.000 0 0 -1 0 0 2
	 1664 1370 1664 2443
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1664 2443 1664 2658
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 805 1675 547 1733
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 57.25 114.51
	 1807 1442 2809 1442
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 8
	 518 1227 662 869 948 654 1234 583 1735 583 2236 726
	 2594 1084 2594 1370
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 0.000
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 11
	 2594 1084 2714 1174 2785 1346 2761 1585 2475 1871 2022 2014
	 1521 2014 1067 1871 709 1585 542 1370 518 1227
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 0.000
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 13
	 2723 1680 2799 1775 2809 1895 2761 2062 2451 2315 2022 2443
	 1521 2443 1091 2300 733 2014 547 1728 504 1585 495 1370
	 538 1322
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 -1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 870 1725 300 $x_3$-axis\001
4 0 0 100 0 0 12 0.0000 2 165 315 2407 2062 $w$\001
4 0 0 100 0 0 12 0.0000 2 195 1650 2475 2467 $u(\\rho,\\theta + 2\\pi)$\001
4 0 0 100 0 0 12 0.0000 2 195 1230 2166 1597 $u(\\rho, \\theta)$\001


==> unot3 <==
#FIG 3.2
Portrait
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 825 300 975 525
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2625 300 2700 525
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1742 390 2042 465
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1515 3000 1515
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 641 3000 641
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1078 3000 1078
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1297 3000 1297
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1406 3000 1406
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1187 3000 1187
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 969 3000 969
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 750 3000 750
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 532 3000 532
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1450 1515 3000 1515
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1550 1406 600 1406
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1575 1297 3000 1297
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1520 1187 600 1187
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1575 1078 3000 1078
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1640 969 600 969
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1725 860 3000 860
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1800 750 600 750
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1950 641 3000 641
2 1 0 3 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2025 532 600 532
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 860 3000 860
3 0 2 1 0 7 100 0 -1 1.500 0 0 0 14
	 1350 1597 1500 1474 1500 1433 1575 1351 1575 1269 1500 1228
	 1575 1105 1575 1024 1725 901 1725 819 1875 696 1875 696
	 2025 573 2100 450
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 1.000 1.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 1620 592 270 One half of $\\Sigma$.\001
4 0 0 100 0 0 12 0.0000 2 135 1095 2310 262 The other half.\001
4 0 0 100 0 0 12 0.0000 2 195 1110 1568 449 $\\mathcal{S}$\001


==> unot3a <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1050 675 437 437 1050 675 1275 1050
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 2550 675 437 437 2550 675 2775 1050
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1425 437 437 1800 1425 2025 1800
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 975 675 1125 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 975 700 1125 700
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 975 650 1125 650
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1425 1375 2175 1375
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2175 700 2925 700
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2175 675 2925 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 2175 650 2925 650
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1629 1041 1941 1041
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1562 1105 2040 1105
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1560 1750 2060 1750
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1505 1710 2085 1710
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1445 1575 2155 1575
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1429 1528 2170 1528
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1485 1670 2115 1670
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1459 1618 2143 1618
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1432 1275 2170 1275
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1466 1225 2139 1225
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1498 1183 2096 1183
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1515 1145 2079 1145
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1425 1330 2175 1330
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1620 1795 1990 1795
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1425 1469 2175 1469
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1425 1420 2175 1420
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1596 1071 2015 1071
4 0 0 100 0 0 12 0.0000 2 135 180 975 1275 A.\001
4 0 0 100 0 0 12 0.0000 2 135 165 1725 2100 C.\001
4 0 0 100 0 0 12 0.0000 2 135 165 2550 1275 B.\001
4 0 0 100 0 0 12 0.0000 2 195 510 1575 427 $B_R$\001


==> unot4 <==
#FIG 3.2
Portrait
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 600 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 1
	 600 2250
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 620 3000 620
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 750 3000 750
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2170 3000 2170
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1800 2400 1800 210
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1510 3000 1510
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1100 3000 1100
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1910 3000 1910
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2100 3000 2100
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 870 3000 870
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 680 3000 680
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 640 3000 640
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 600 3000 600
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2390 3000 2390
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2400 3000 2400
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2250 3000 2250
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2325 3000 2325
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 2360 3000 2360
4 0 0 100 0 0 12 0.0000 2 195 870 1875 300 $x_3$-axis\001
4 0 0 100 0 0 12 0.0000 2 195 495 3075 645 $\\pi/2$\001
4 0 0 100 0 0 12 0.0000 2 195 600 3083 2460 $-\\pi/2$\001
4 0 0 100 0 0 12 0.0000 2 180 1365 3068 1186 Spiraling into both\001
4 0 0 100 0 0 12 0.0000 2 195 960 3060 1395 $x_3 = \\pi/2$\001
4 0 0 100 0 0 12 0.0000 2 195 1110 3060 1598 $x_3 = -\\pi/2$.\001


==> unot5 <==
#FIG 3.2
Portrait
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 2400 1900 1000 1000 2400 1900 3400 1900
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 2400 1900 500 500 2400 1900 2900 1900
1 3 0 1 0 7 100 0 -1 0.000 1 0.0000 2400 1900 60 60 2400 1900 2460 1900
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1900 4200 1900
3 2 0 1 0 7 100 0 -1 0.000 0 0 0 28
	 1575 1350 1650 1350 1650 1425 1725 1425 1725 1575 1800 1575
	 1875 1650 1950 1650 2025 1725 2025 1725 2100 1800 2175 1800
	 2325 1875 2325 1875 2400 1875 2400 1875 2550 1800 2550 1800
	 2550 1800 2625 1800 2775 1800 2850 1800 3000 1800 3150 1725
	 3225 1650 3225 1650 3300 1650 3375 1725
	 0.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000 -1.000
	 -1.000 -1.000 -1.000 0.000
4 0 0 100 0 0 12 0.0000 2 195 690 1792 1417 $\\Sigma$\001
4 0 0 100 0 0 12 0.0000 2 195 1440 2250 2122 $B_{\\epsilon r_0}$\001
4 0 0 100 0 0 12 0.0000 2 195 810 2641 2505 $B_{r_0}$\001
4 0 0 100 0 0 12 0.0000 2 195 900 3037 2827 $B_{2r_0}$\001
4 0 0 100 0 0 12 0.0000 2 195 735 3901 2077 $x_3 = 0$\001


==> unot7 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2325 900 2325 1200
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 600 1450 3000 1450
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 600 1380 1400 1380 1900 1350 1400 1320 600 1320
	 0.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 5
	 3000 1380 2200 1380 1700 1350 2200 1320 3000 1320
	 0.000 1.000 1.000 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 135 1440 1657 863 Rescaled catenoid.\001
4 0 0 100 0 0 12 0.0000 2 195 735 2309 1635 $x_3 = 0$\001


==> unot8 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 675 675 225 1800 675 1125 450
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 1800 1725 675 225 1800 1725 1125 1500
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 675 2475 1725
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 0 0 2
	 1125 1725 2475 675
2 1 0 1 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2400 375 2175 600
3 0 0 1 0 7 100 0 -1 0.000 0 0 0 18
	 1950 1725 1800 1575 1800 1425 1800 1350 1800 1275 1800 1050
	 1800 825 1725 750 1800 675 1800 600 1800 525 1800 525
	 1725 450 1725 375 1650 375 1650 300 1650 225 1575 150
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 1.000 0.000
4 0 0 100 0 0 12 0.0000 2 165 270 1935 1275 $x$\001
4 0 0 100 0 0 12 0.0000 2 195 1110 1297 323 $\\mathcal{S}$\001
4 0 0 100 0 0 12 0.0000 2 195 1515 2212 278 $\\cone_{\\delta}(x)$\001

